Is AUC the best measure for practical comparison of anomaly detectors?

The area under receiver operating characteristics (AUC) is the standard measure for comparison of anomaly detectors. Its advantage is in providing a scalar number that allows a natural ordering and is independent on a threshold, which allows to postpone the choice. In this work, we question whether AUC is a good metric for anomaly detection, or if it gives a false sense of comfort, due to relying on assumptions which are unlikely to hold in practice. Our investigation shows that variations of AUC emphasizing accuracy at low false positive rate seem to be better correlated with the needs of practitioners, but also that we can compare anomaly detectors only in the case when we have representative examples of anomalous samples. This last result is disturbing, as it suggests that in many cases, we should do active or few-show learning instead of pure anomaly detection.

==> Measure Evaluation/table_confusion_example.tex <==
\begin{table}
\centering
	\begin{tabular}{c | c c}
		true label/estimated label & normal & anomalous \\
		\hline
		normal & tn & fp  \\
		anomalous & fn & tp 
	\end{tabular}
	\caption{A confusion matrix of a model.}
	\label{tab:conf_ex}
\end{table}

==> Measure Evaluation/table_hyperparams.tex <==
\begin{table}
	\centering
	\begin{tabular}{c | c c}
		algorithm & hyperparameter & values \\
		\hline
		kNN & distance & $\lbrace \kappa(x), \gamma(x), \delta(x) \rbrace$  \\
		    & k & $\lbrace 1, 3, 5, 7, 9, 13, 21, 31, 51 \rbrace$ \\
		LOF & k & $\lbrace 10, 20, 50 \rbrace$ \\
		IF & $N_t$ & $\lbrace 50, 100, 200 \rbrace$ \\
		OCSVM & $\gamma$ &$\lbrace 0.01, 0.05, 0.1, 0.5, 1, 5, 10, 50, 100 \rbrace$ \\
	\end{tabular}
	\caption{Overview of used hyperparameter values.}
	\label{tab:hyperparams}
\end{table}


==> Measure Evaluation/table_measure_comparison_full_0_by_models.tex <==
\begin{table*} 
 \center 
 \resizebox{\textwidth}{!}{ 
 \begin{tabular}[h]{c c c c c c c c c c c c c c c } 
  max/loss & \rotatebox{90}{AUC} & \rotatebox{90}{AUC$_w$} & \rotatebox{90}{AUC@0.05} & \rotatebox{90}{AUC@0.01} & \rotatebox{90}{precision@0.05} & \rotatebox{90}{precision@0.01} & \rotatebox{90}{TPR@0.05} & \rotatebox{90}{TPR@0.01} & \rotatebox{90}{F1@0.05} & \rotatebox{90}{F1@0.01} & \rotatebox{90}{CVOL@0.05} & \rotatebox{90}{CVOL@0.01} & \rotatebox{90}{} & \rotatebox{90}{mean}  \\ 
  \hline 
  AUC & -- & \cellcolor{gray!30}0.4\% & 1.2\% & 2.0\% & 2.0\% & 2.3\% & \cellcolor{gray!15}1.0\% & 2.4\% & 7.1\% & 10.9\% & 3.7\% & 8.9\% &  & 3.5\%  \\ 
  AUC$_w$ & \cellcolor{gray!45}0.1\% & -- & \cellcolor{gray!45}0.5\% & 1.3\% & \cellcolor{gray!15}1.7\% & \cellcolor{gray!30}1.6\% & \cellcolor{gray!30}0.6\% & 1.6\% & 6.7\% & 10.3\% & 3.6\% & 9.7\% &  & 3.1\%  \\ 
  AUC@0.05 & \cellcolor{gray!30}0.3\% & \cellcolor{gray!45}0.2\% & -- & \cellcolor{gray!30}0.7\% & \cellcolor{gray!45}1.5\% & 1.8\% & \cellcolor{gray!45}0.4\% & \cellcolor{gray!30}0.9\% & \cellcolor{gray!30}5.3\% & 8.4\% & 1.9\% & 8.0\% &  & \cellcolor{gray!45}2.4\%  \\ 
  AUC@0.01 & 0.7\% & 0.8\% & \cellcolor{gray!15}1.0\% & -- & 2.5\% & \cellcolor{gray!45}1.4\% & 2.1\% & \cellcolor{gray!45}0.5\% & 6.3\% & \cellcolor{gray!30}7.9\% & 1.7\% & \cellcolor{gray!15}5.1\% &  & \cellcolor{gray!30}2.5\%  \\ 
  precision@0.05 & 0.5\% & \cellcolor{gray!15}0.7\% & 1.0\% & 2.3\% & -- & 2.4\% & 1.3\% & 2.2\% & 6.6\% & 10.1\% & \cellcolor{gray!15}1.5\% & 7.1\% &  & 3.0\%  \\ 
  precision@0.01 & 0.7\% & 1.0\% & 1.5\% & \cellcolor{gray!15}0.7\% & \cellcolor{gray!30}1.6\% & -- & 2.8\% & \cellcolor{gray!15}1.4\% & 10.1\% & 12.5\% & \cellcolor{gray!45}0.0\% & \cellcolor{gray!45}1.9\% &  & 2.9\%  \\ 
  TPR@0.05 & \cellcolor{gray!15}0.3\% & 1.5\% & 1.9\% & 5.7\% & 2.2\% & 4.6\% & -- & 4.5\% & 6.2\% & 12.3\% & 3.1\% & 9.2\% &  & 4.3\%  \\ 
  TPR@0.01 & 0.6\% & 1.1\% & \cellcolor{gray!30}1.0\% & \cellcolor{gray!45}0.5\% & 2.3\% & \cellcolor{gray!15}1.8\% & 2.2\% & -- & \cellcolor{gray!15}6.2\% & \cellcolor{gray!15}8.2\% & 1.7\% & 8.4\% &  & \cellcolor{gray!15}2.8\%  \\ 
  F1@0.05 & 3.6\% & 11.0\% & 10.3\% & 13.1\% & 14.0\% & 21.2\% & 8.8\% & 12.4\% & -- & \cellcolor{gray!45}6.0\% & 1.7\% & 12.1\% &  & 9.5\%  \\ 
  F1@0.01 & 3.5\% & 17.7\% & 16.9\% & 27.7\% & 13.8\% & 37.1\% & 10.1\% & 24.5\% & \cellcolor{gray!45}3.4\% & -- & 1.5\% & \cellcolor{gray!30}3.1\% &  & 13.3\%  \\ 
  CVOL@0.05 & 3.8\% & 13.3\% & 18.1\% & 22.1\% & 18.7\% & 15.8\% & 15.9\% & 19.7\% & 9.5\% & 22.0\% & -- & 14.4\% &  & 14.4\%  \\ 
  CVOL@0.01 & 1.4\% & 6.4\% & 7.0\% & 12.0\% & 6.5\% & 9.3\% & 5.9\% & 7.7\% & 7.9\% & 9.2\% & \cellcolor{gray!30}0.2\% & -- &  & 6.1\%  \\ 
 \end{tabular}
 }
 \caption{Means of relative loss in a column measure when optimal model and hyperparameters are selected using the row measure. 0\%  training contamination. Level of shading highlights three best results in a column.} 
 \label{tab:measure_comparison_full_0_by_models} 
\end{table*}

==> Measure Evaluation/table_measure_comparison_full_1_by_models.tex <==
\begin{table*} 
 \center 
 \resizebox{\textwidth}{!}{ 
 \begin{tabular}[h]{c c c c c c c c c c c c c c c } 
  max/loss & \rotatebox{90}{AUC} & \rotatebox{90}{AUC$_w$} & \rotatebox{90}{AUC@0.05} & \rotatebox{90}{AUC@0.01} & \rotatebox{90}{precision@0.05} & \rotatebox{90}{precision@0.01} & \rotatebox{90}{TPR@0.05} & \rotatebox{90}{TPR@0.01} & \rotatebox{90}{F1@0.05} & \rotatebox{90}{F1@0.01} & \rotatebox{90}{CVOL@0.05} & \rotatebox{90}{CVOL@0.01} & \rotatebox{90}{} & \rotatebox{90}{mean}  \\ 
  \hline 
  AUC & -- & 1.2\% & 2.1\% & 5.1\% & 2.5\% & 3.5\% & \cellcolor{gray!15}1.3\% & 4.3\% & 8.1\% & 13.1\% & 4.1\% & 10.1\% &  & 4.6\%  \\ 
  AUC$_w$ & \cellcolor{gray!45}0.2\% & -- & \cellcolor{gray!45}0.6\% & 1.2\% & \cellcolor{gray!30}1.9\% & \cellcolor{gray!15}1.2\% & \cellcolor{gray!30}1.1\% & 1.6\% & 7.6\% & 11.1\% & 4.1\% & 10.4\% &  & 3.4\%  \\ 
  AUC@0.05 & 0.7\% & \cellcolor{gray!45}0.4\% & -- & \cellcolor{gray!30}0.7\% & \cellcolor{gray!45}1.8\% & \cellcolor{gray!30}1.1\% & \cellcolor{gray!45}0.9\% & \cellcolor{gray!30}0.9\% & \cellcolor{gray!30}6.2\% & 9.5\% & 2.4\% & 9.7\% &  & \cellcolor{gray!30}2.9\%  \\ 
  AUC@0.01 & 0.9\% & \cellcolor{gray!30}0.8\% & \cellcolor{gray!30}0.8\% & -- & 2.3\% & \cellcolor{gray!45}1.0\% & 2.2\% & \cellcolor{gray!45}0.5\% & 7.1\% & \cellcolor{gray!30}8.7\% & 2.2\% & \cellcolor{gray!15}6.3\% &  & \cellcolor{gray!45}2.7\%  \\ 
  precision@0.05 & \cellcolor{gray!15}0.5\% & \cellcolor{gray!15}1.0\% & 1.5\% & 3.2\% & -- & 2.3\% & 1.4\% & 2.7\% & 7.5\% & 11.7\% & 2.1\% & 7.5\% &  & 3.5\%  \\ 
  precision@0.01 & 1.2\% & 1.3\% & 1.7\% & \cellcolor{gray!15}1.2\% & \cellcolor{gray!15}2.1\% & -- & 3.1\% & \cellcolor{gray!15}1.4\% & 11.2\% & 14.2\% & \cellcolor{gray!45}0.1\% & \cellcolor{gray!45}3.9\% &  & 3.4\%  \\ 
  TPR@0.05 & \cellcolor{gray!30}0.4\% & 2.2\% & 2.5\% & 7.9\% & 2.4\% & 5.2\% & -- & 6.1\% & \cellcolor{gray!15}6.7\% & 13.6\% & 3.5\% & 8.9\% &  & 4.9\%  \\ 
  TPR@0.01 & 0.9\% & 1.2\% & \cellcolor{gray!15}0.9\% & \cellcolor{gray!45}0.6\% & 2.6\% & 1.3\% & 2.5\% & -- & 7.1\% & \cellcolor{gray!15}9.0\% & 2.1\% & 9.6\% &  & \cellcolor{gray!15}3.2\%  \\ 
  F1@0.05 & 4.5\% & 12.6\% & 10.8\% & 13.7\% & 16.5\% & 19.3\% & 10.2\% & 12.6\% & -- & \cellcolor{gray!45}6.2\% & 2.0\% & 11.2\% &  & 10.0\%  \\ 
  F1@0.01 & 7.2\% & 21.9\% & 21.3\% & 19.3\% & 27.2\% & 33.6\% & 22.7\% & 20.7\% & \cellcolor{gray!45}4.3\% & -- & \cellcolor{gray!15}1.9\% & \cellcolor{gray!30}4.3\% &  & 15.4\%  \\ 
  CVOL@0.05 & 4.6\% & 17.5\% & 24.2\% & 31.3\% & 20.5\% & 23.8\% & 20.0\% & 27.6\% & 12.6\% & 27.3\% & -- & 14.1\% &  & 18.6\%  \\ 
  CVOL@0.01 & 3.3\% & 14.8\% & 19.0\% & 26.3\% & 14.0\% & 23.7\% & 15.1\% & 22.6\% & 13.7\% & 18.7\% & \cellcolor{gray!30}0.2\% & -- &  & 14.3\%  \\ 
 \end{tabular}
 }
 \caption{Means of relative loss in a column measure when optimal model and hyperparameters are selected using the row measure. 1\% contamination.} 
 \label{tab:measure_comparison_full_1_by_models} 
\end{table*}

==> Measure Evaluation/table_measure_comparison_full_5_by_models.tex <==
\begin{table*} 
 \center 
 \resizebox{\textwidth}{!}{ 
 \begin{tabular}[h]{c c c c c c c c c c c c c c c } 
  max/loss & \rotatebox{90}{AUC} & \rotatebox{90}{AUC$_w$} & \rotatebox{90}{AUC@0.05} & \rotatebox{90}{AUC@0.01} & \rotatebox{90}{precision@0.05} & \rotatebox{90}{precision@0.01} & \rotatebox{90}{TPR@0.05} & \rotatebox{90}{TPR@0.01} & \rotatebox{90}{F1@0.05} & \rotatebox{90}{F1@0.01} & \rotatebox{90}{CVOL@0.05} & \rotatebox{90}{CVOL@0.01} & \rotatebox{90}{} & \rotatebox{90}{mean}  \\ 
  \hline 
  AUC & -- & \cellcolor{gray!15}1.3\% & 3.2\% & 5.4\% & 2.7\% & 5.1\% & 1.9\% & 5.2\% & 10.8\% & 21.2\% & 4.0\% & 9.7\% &  & 5.9\%  \\ 
  AUC$_w$ & \cellcolor{gray!45}0.3\% & -- & \cellcolor{gray!45}0.8\% & 1.7\% & \cellcolor{gray!45}1.8\% & \cellcolor{gray!45}1.5\% & \cellcolor{gray!30}1.0\% & 1.9\% & 9.7\% & 18.3\% & 3.3\% & 8.3\% &  & \cellcolor{gray!30}4.1\%  \\ 
  AUC@0.05 & 0.8\% & \cellcolor{gray!45}0.6\% & -- & \cellcolor{gray!30}1.6\% & \cellcolor{gray!30}1.9\% & \cellcolor{gray!30}1.8\% & \cellcolor{gray!45}0.9\% & \cellcolor{gray!30}1.1\% & \cellcolor{gray!15}8.4\% & 17.2\% & 2.2\% & 9.0\% &  & \cellcolor{gray!45}3.8\%  \\ 
  AUC@0.01 & 1.9\% & 2.2\% & \cellcolor{gray!15}1.6\% & -- & 3.8\% & \cellcolor{gray!15}2.0\% & 3.7\% & \cellcolor{gray!45}0.3\% & 10.5\% & \cellcolor{gray!30}16.1\% & 1.9\% & \cellcolor{gray!15}6.5\% &  & \cellcolor{gray!15}4.2\%  \\ 
  precision@0.05 & \cellcolor{gray!15}0.6\% & \cellcolor{gray!30}0.9\% & 1.6\% & 3.3\% & -- & 2.4\% & \cellcolor{gray!15}1.3\% & 3.0\% & 9.6\% & 19.4\% & 2.0\% & 6.9\% &  & 4.3\%  \\ 
  precision@0.01 & 2.3\% & 2.6\% & 1.8\% & \cellcolor{gray!15}1.6\% & 2.9\% & -- & 4.2\% & \cellcolor{gray!15}1.5\% & 15.3\% & 24.5\% & \cellcolor{gray!45}0.1\% & \cellcolor{gray!45}2.8\% &  & 5.0\%  \\ 
  TPR@0.05 & \cellcolor{gray!30}0.6\% & 1.5\% & 2.0\% & 5.6\% & \cellcolor{gray!15}2.1\% & 4.6\% & -- & 4.6\% & \cellcolor{gray!30}8.2\% & 19.3\% & 2.7\% & 7.7\% &  & 4.9\%  \\ 
  TPR@0.01 & 1.6\% & 2.1\% & \cellcolor{gray!30}1.5\% & \cellcolor{gray!45}0.5\% & 3.9\% & 2.3\% & 3.7\% & -- & 10.4\% & \cellcolor{gray!15}16.2\% & \cellcolor{gray!15}1.9\% & 8.0\% &  & 4.3\%  \\ 
  F1@0.05 & 7.8\% & 19.4\% & 16.2\% & 16.0\% & 26.2\% & 28.9\% & 17.5\% & 16.0\% & -- & \cellcolor{gray!45}6.9\% & 1.9\% & 10.6\% &  & 14.0\%  \\ 
  F1@0.01 & 12.6\% & 32.9\% & 29.9\% & 24.6\% & 39.3\% & 50.8\% & 32.9\% & 27.4\% & \cellcolor{gray!45}5.1\% & -- & 1.9\% & \cellcolor{gray!30}4.8\% &  & 21.9\%  \\ 
  CVOL@0.05 & 8.5\% & 26.4\% & 36.5\% & 41.1\% & 27.9\% & 38.5\% & 32.7\% & 39.2\% & 23.9\% & 41.4\% & -- & 12.5\% &  & 27.4\%  \\ 
  CVOL@0.01 & 8.0\% & 25.1\% & 34.0\% & 37.4\% & 23.8\% & 43.9\% & 30.6\% & 36.8\% & 26.8\% & 36.8\% & \cellcolor{gray!30}0.3\% & -- &  & 25.3\%  \\ 
 \end{tabular}
 }
 \caption{Means of relative performance loss in a column measure when optimal model and hyperparameters are selected using the row measure. 5\% training contamination.} 
 \label{tab:measure_comparison_full_5_by_models} 
\end{table*}

==> Measure Evaluation/table_measure_correlation_full_0.tex <==
\begin{table*} 
 \center 
 \begin{tabular}[h]{c c c c c c c c c c c c c c c } 
  measure & \rotatebox{90}{AUC} & \rotatebox{90}{AUC$_w$} & \rotatebox{90}{AUC@0.05} & \rotatebox{90}{AUC@0.01} & \rotatebox{90}{precision@0.05} & \rotatebox{90}{precision@0.01} & \rotatebox{90}{TPR@0.05} & \rotatebox{90}{TPR@0.01} & \rotatebox{90}{F1@0.05} & \rotatebox{90}{F1@0.01} & \rotatebox{90}{CVOL@0.05} & \rotatebox{90}{CVOL@0.01} & \rotatebox{90}{} & \rotatebox{90}{mean}  \\ 
  \hline 
  AUC & -- & \cellcolor{gray!45}0.84 & 0.77 & 0.67 & \cellcolor{gray!15}0.75 & 0.63 & 0.69 & 0.65 & 0.62 & 0.59 & 0.42 & 0.46 &  & 0.67  \\ 
  AUC$_w$ & \cellcolor{gray!45}0.84 & -- & \cellcolor{gray!30}0.82 & 0.75 & \cellcolor{gray!30}0.76 & \cellcolor{gray!15}0.70 & 0.68 & 0.70 & 0.62 & 0.63 & 0.42 & 0.49 &  & 0.70  \\ 
  AUC@0.05 & \cellcolor{gray!30}0.77 & \cellcolor{gray!30}0.82 & -- & \cellcolor{gray!30}0.83 & \cellcolor{gray!45}0.77 & \cellcolor{gray!45}0.72 & \cellcolor{gray!30}0.78 & \cellcolor{gray!15}0.82 & \cellcolor{gray!30}0.72 & \cellcolor{gray!15}0.73 & 0.47 & 0.55 &  & \cellcolor{gray!45}0.75  \\ 
  AUC@0.01 & 0.67 & 0.75 & \cellcolor{gray!45}0.83 & -- & 0.68 & \cellcolor{gray!30}0.70 & 0.64 & \cellcolor{gray!45}0.89 & 0.61 & \cellcolor{gray!30}0.78 & 0.43 & 0.57 &  & \cellcolor{gray!15}0.71  \\ 
  precision@0.05 & \cellcolor{gray!15}0.75 & \cellcolor{gray!15}0.76 & 0.77 & 0.68 & -- & 0.65 & \cellcolor{gray!15}0.70 & 0.68 & 0.65 & 0.63 & 0.44 & 0.49 &  & 0.68  \\ 
  precision@0.01 & 0.63 & 0.70 & 0.72 & 0.70 & 0.65 & -- & 0.56 & 0.67 & 0.47 & 0.57 & 0.32 & 0.44 &  & 0.62  \\ 
  TPR@0.05 & 0.69 & 0.68 & 0.78 & 0.64 & 0.70 & 0.56 & -- & 0.67 & \cellcolor{gray!45}0.91 & 0.61 & 0.48 & 0.47 &  & 0.68  \\ 
  TPR@0.01 & 0.65 & 0.70 & \cellcolor{gray!15}0.82 & \cellcolor{gray!45}0.89 & 0.68 & 0.67 & 0.67 & -- & 0.63 & \cellcolor{gray!45}0.88 & 0.45 & \cellcolor{gray!15}0.60 &  & \cellcolor{gray!30}0.72  \\ 
  F1@0.05 & 0.62 & 0.62 & 0.72 & 0.61 & 0.65 & 0.47 & \cellcolor{gray!45}0.91 & 0.63 & -- & 0.67 & \cellcolor{gray!30}0.54 & 0.52 &  & 0.66  \\ 
  F1@0.01 & 0.59 & 0.63 & 0.73 & \cellcolor{gray!15}0.78 & 0.63 & 0.57 & 0.61 & \cellcolor{gray!30}0.88 & \cellcolor{gray!15}0.67 & -- & \cellcolor{gray!15}0.48 & \cellcolor{gray!45}0.70 &  & 0.69  \\ 
  CVOL@0.05 & 0.42 & 0.42 & 0.47 & 0.43 & 0.44 & 0.32 & 0.48 & 0.45 & 0.54 & 0.48 & -- & \cellcolor{gray!30}0.64 &  & 0.51  \\ 
  CVOL@0.01 & 0.46 & 0.49 & 0.55 & 0.57 & 0.49 & 0.44 & 0.47 & 0.60 & 0.52 & 0.70 & \cellcolor{gray!45}0.64 & -- &  & 0.58  \\ 
 \end{tabular}
 \caption{Average of Kendall correlation between measures over datasets, 0\% contamination. Level of shading highlights three highest correlations in a column.} 
 \label{tab:measure_correlation_full_0} 
\end{table*}

==> Measure Evaluation/table_model_ranks_0.tex <==
\begin{table} 
 \center 
 \begin{tabular}[h]{c c c c c } 
  measure & kNN & LOF & IF & OCSVM  \\ 
  \hline 
  AUC & 1.56$\pm$0.72 & 2.81$\pm$1.00 & 3.55$\pm$0.79 & 2.09$\pm$0.72  \\ 
  AUC$_w$ & 1.60$\pm$0.74 & 2.69$\pm$1.05 & 3.56$\pm$0.81 & 2.15$\pm$0.73  \\ \rule{0pt}{1.5em}
  AUC@0.05 & 1.51$\pm$0.71 & 2.72$\pm$1.05 & 3.56$\pm$0.79 & 2.21$\pm$0.65  \\ 
  precision@0.05 & 1.51$\pm$0.69 & 2.64$\pm$1.00 & 3.55$\pm$0.86 & 2.30$\pm$0.72  \\ 
  TPR@0.05 & 1.68$\pm$0.73 & 2.72$\pm$0.95 & 3.51$\pm$0.84 & 2.09$\pm$0.64  \\ 
  F1@0.05 & 1.80$\pm$0.74 & 2.78$\pm$0.90 & 3.55$\pm$0.78 & 1.87$\pm$0.69  \\ 
  CVOL@0.05 & 1.65$\pm$0.43 & 3.19$\pm$0.60 & 3.64$\pm$0.60 & 1.53$\pm$0.43  \\ \rule{0pt}{1.5em}
  AUC@0.01 & 1.58$\pm$0.71 & 2.63$\pm$1.09 & 3.59$\pm$0.74 & 2.20$\pm$0.73  \\ 
  precision@0.01 & 2.22$\pm$1.25 & 2.32$\pm$0.84 & 2.94$\pm$1.36 & 2.51$\pm$0.68  \\ 
  TPR@0.01 & 1.52$\pm$0.59 & 2.72$\pm$0.98 & 3.64$\pm$0.69 & 2.12$\pm$0.78  \\ 
  F1@0.01 & 1.76$\pm$0.70 & 2.86$\pm$0.80 & 3.70$\pm$0.59 & 1.68$\pm$0.77  \\ 
  CVOL@0.01 & 1.85$\pm$0.68 & 3.20$\pm$0.61 & 3.59$\pm$0.66 & 1.36$\pm$0.47  \\ 
 \end{tabular}
 \caption{Means and standard deviations of algorithm ranks using different measures, 0\% training contamination.} 
 \label{tab:model_ranks_0} 
\end{table}

==> Measure Evaluation/table_model_ranks_umap.tex <==
\begin{table} 
 \center 
 \begin{tabular}[h]{c c c c c } 
  measure & kNN & LOF & IF & OCSVM  \\ 
  \hline 
  AUC & 1.52$\pm$0.64 & 2.98$\pm$0.78 & 3.60$\pm$0.71 & 1.91$\pm$0.57  \\ 
  AUC$_w$ & 1.56$\pm$0.77 & 3.00$\pm$0.69 & 3.66$\pm$0.71 & 1.78$\pm$0.54  \\  \rule{0pt}{1.5em}
  AUC@0.05 & 1.55$\pm$0.64 & 2.90$\pm$0.73 & 3.70$\pm$0.60 & 1.85$\pm$0.59  \\ 
  precision@0.05 & 1.51$\pm$0.70 & 2.90$\pm$0.71 & 3.57$\pm$0.70 & 2.02$\pm$0.54  \\ 
  TPR@0.05 & 1.61$\pm$0.70 & 2.87$\pm$0.68 & 3.42$\pm$0.74 & 2.11$\pm$0.54  \\ 
  CVOL@0.05 & 1.20$\pm$0.40 & 2.96$\pm$0.61 & 3.82$\pm$0.40 & 2.01$\pm$0.65  \\  \rule{0pt}{1.5em}
  AUC@0.01 & 1.54$\pm$0.57 & 2.92$\pm$0.70 & 3.71$\pm$0.59 & 1.84$\pm$0.58  \\ 
  precision@0.01 & 2.16$\pm$1.12 & 2.61$\pm$0.71 & 3.04$\pm$1.25 & 2.19$\pm$0.65  \\ 
  TPR@0.01 & 1.56$\pm$0.57 & 2.86$\pm$0.72 & 3.73$\pm$0.55 & 1.85$\pm$0.58  \\ 
  CVOL@0.01 & 1.39$\pm$0.65 & 2.96$\pm$0.56 & 3.81$\pm$0.45 & 1.83$\pm$0.68  \\ \hline
 \end{tabular}
 \caption{Means and standard deviations of algorithm ranks using different measures, UMAP datasets, 0\% training contamination.} 
 \label{tab:model_ranks_umap} 
\end{table}

==> Measure Evaluation/table_model_ranks_umap_0.tex <==
\begin{table} 
 \center 
 \begin{tabular}[h]{c c c c c } 
  measure & kNN & LOF & IF & OCSVM  \\ 
  \hline 
  AUC & 1.53$\pm$0.64 & 2.96$\pm$0.77 & 3.61$\pm$0.72 & 1.90$\pm$0.57  \\ 
  AUC$_w$ & 1.49$\pm$0.61 & 3.02$\pm$0.64 & 3.68$\pm$0.68 & 1.81$\pm$0.56  \\ \rule{0pt}{1.5em}
  AUC@0.05 & 1.55$\pm$0.64 & 2.87$\pm$0.70 & 3.72$\pm$0.62 & 1.86$\pm$0.59  \\ 
  precision@0.05 & 1.49$\pm$0.74 & 2.93$\pm$0.67 & 3.61$\pm$0.72 & 1.96$\pm$0.50  \\ 
  TPR@0.05 & 1.60$\pm$0.69 & 2.85$\pm$0.67 & 3.44$\pm$0.73 & 2.11$\pm$0.55  \\ 
  F1@0.05 & 1.61$\pm$0.68 & 2.84$\pm$0.68 & 3.45$\pm$0.72 & 2.10$\pm$0.56  \\ 
  CVOL@0.05 & 1.21$\pm$0.41 & 2.95$\pm$0.60 & 3.84$\pm$0.39 & 2.01$\pm$0.65  \\ \rule{0pt}{1.5em}
  AUC@0.01 & 1.54$\pm$0.57 & 2.90$\pm$0.68 & 3.72$\pm$0.63 & 1.85$\pm$0.59  \\ 
  precision@0.01 & 2.11$\pm$1.16 & 2.64$\pm$0.72 & 3.08$\pm$1.25 & 2.17$\pm$0.69  \\ 
  TPR@0.01 & 1.57$\pm$0.58 & 2.85$\pm$0.71 & 3.71$\pm$0.60 & 1.87$\pm$0.60  \\ 
  F1@0.01 & 1.57$\pm$0.58 & 2.82$\pm$0.70 & 3.72$\pm$0.60 & 1.89$\pm$0.60  \\ 
  CVOL@0.01 & 1.38$\pm$0.64 & 2.96$\pm$0.58 & 3.81$\pm$0.45 & 1.85$\pm$0.68  \\ 
 \end{tabular}
 \caption{Means and standard deviations of algorithm ranks using different measures, UMAP datasets, 0\% training contamination.} 
 \label{tab:model_ranks_umap_0} 
\end{table}

==> Measure Evaluation/table_multiclass_all_means_full_0.tex <==
\begin{table} 
 \center 
 \begin{tabular}[h]{c c c c c c c c } 
  measure & \rotatebox{90}{AUC} & \rotatebox{90}{AUC$_w$} & \rotatebox{90}{AUC@0.05} & \rotatebox{90}{precision@0.05} & \rotatebox{90}{TPR@0.05} & \rotatebox{90}{F1@0.05} & \rotatebox{90}{CVOL@0.05}  \\ 
  \hline 
  AUC & \cellcolor{gray!45}0.8\% & \cellcolor{gray!45}2.4\% & 6.3\% & 5.8\% & 4.8\% & 8.2\% & 3.3\%  \\ 
  AUC$_w$ & \cellcolor{gray!30}0.9\% & \cellcolor{gray!15}2.5\% & 6.2\% & 5.8\% & \cellcolor{gray!15}4.6\% & 8.2\% & 3.3\%  \\ 
  AUC@0.05 & 0.9\% & \cellcolor{gray!30}2.5\% & \cellcolor{gray!45}5.0\% & \cellcolor{gray!15}5.4\% & \cellcolor{gray!30}4.0\% & \cellcolor{gray!30}5.9\% & 1.4\%  \\ 
  precision@0.05 & 0.9\% & 2.7\% & \cellcolor{gray!15}6.0\% & \cellcolor{gray!45}4.3\% & 4.9\% & 6.8\% & \cellcolor{gray!30}1.0\%  \\ 
  TPR@0.05 & \cellcolor{gray!15}0.9\% & 2.9\% & \cellcolor{gray!30}5.7\% & \cellcolor{gray!30}5.2\% & \cellcolor{gray!45}3.7\% & 7.1\% & 2.1\%  \\ 
  F1@0.05 & 2.5\% & 10.2\% & 14.2\% & 14.6\% & 10.6\% & \cellcolor{gray!45}4.0\% & \cellcolor{gray!15}1.2\%  \\ 
  CVOL@0.05 & 2.3\% & 9.0\% & 13.8\% & 15.2\% & 11.6\% & \cellcolor{gray!15}6.6\% & \cellcolor{gray!45}0.4\%  \\ 
 \end{tabular}
 \caption{All full datasets, mean of multiclass sensitivities, 0\% training contamination.} 
 \label{tab:multiclass_all_means_full_0} 
\end{table}

==> Measure Evaluation/table_multiclass_all_means_umap_0.tex <==
\begin{table} 
 \center 
 \begin{tabular}[h]{c c c c c c c c } 
  measure & \rotatebox{90}{AUC} & \rotatebox{90}{AUC$_w$} & \rotatebox{90}{AUC@0.05} & \rotatebox{90}{precision@0.05} & \rotatebox{90}{TPR@0.05} & \rotatebox{90}{F1@0.05} & \rotatebox{90}{CVOL@0.05}  \\ 
  \hline 
  AUC & 2.0\% & 3.9\% & 6.5\% & 5.4\% & 5.3\% & 4.6\% & 5.2\%  \\ 
  AUC$_w$ & \cellcolor{gray!30}1.6\% & \cellcolor{gray!30}2.8\% & \cellcolor{gray!30}4.7\% & \cellcolor{gray!30}4.2\% & \cellcolor{gray!30}4.2\% & \cellcolor{gray!30}3.4\% & \cellcolor{gray!15}4.4\%  \\ 
  AUC@0.05 & 1.7\% & \cellcolor{gray!15}3.1\% & \cellcolor{gray!15}4.8\% & \cellcolor{gray!15}4.6\% & 4.5\% & 3.7\% & \cellcolor{gray!30}4.3\%  \\ 
  precision@0.05 & 1.8\% & 3.4\% & 5.7\% & 4.8\% & 4.8\% & 3.9\% & 4.7\%  \\ 
  TPR@0.05 & \cellcolor{gray!15}1.7\% & 3.8\% & 6.5\% & 5.0\% & \cellcolor{gray!15}4.2\% & 3.5\% & 4.9\%  \\ 
  F1@0.05 & 1.7\% & 3.8\% & 6.4\% & 5.0\% & 4.2\% & \cellcolor{gray!15}3.5\% & 4.9\%  \\ 
  CVOL@0.05 & \cellcolor{gray!45}1.4\% & \cellcolor{gray!45}2.4\% & \cellcolor{gray!45}3.8\% & \cellcolor{gray!45}3.9\% & \cellcolor{gray!45}4.0\% & \cellcolor{gray!45}3.4\% & \cellcolor{gray!45}0.2\%  \\ 
 \end{tabular}
 \caption{All UMAP datasets, mean of multiclass sensitivities, 0\% training contamination.} 
 \label{tab:multiclass_all_means_umap_0} 
\end{table}

==> table_model_ranks_umap.tex <==
\begin{table} 
 \center 
 \begin{tabular}[h]{c c c c c } 
  measure & kNN & LOF & IF & OCSVM  \\ 
  \hline 
  AUC & 1.52$\pm$0.64 & 2.98$\pm$0.78 & 3.60$\pm$0.71 & 1.91$\pm$0.57  \\ 
  AUC$_w$ & 1.56$\pm$0.77 & 3.00$\pm$0.69 & 3.66$\pm$0.71 & 1.78$\pm$0.54  \\  \rule{0pt}{1.5em}
  AUC@0.05 & 1.55$\pm$0.64 & 2.90$\pm$0.73 & 3.70$\pm$0.60 & 1.85$\pm$0.59  \\ 
  precision@0.05 & 1.51$\pm$0.70 & 2.90$\pm$0.71 & 3.57$\pm$0.70 & 2.02$\pm$0.54  \\ 
  TPR@0.05 & 1.61$\pm$0.70 & 2.87$\pm$0.68 & 3.42$\pm$0.74 & 2.11$\pm$0.54  \\ 
  CVOL@0.05 & 1.20$\pm$0.40 & 2.96$\pm$0.61 & 3.82$\pm$0.40 & 2.01$\pm$0.65  \\  \rule{0pt}{1.5em}
  AUC@0.01 & 1.54$\pm$0.57 & 2.92$\pm$0.70 & 3.71$\pm$0.59 & 1.84$\pm$0.58  \\ 
  precision@0.01 & 2.16$\pm$1.12 & 2.61$\pm$0.71 & 3.04$\pm$1.25 & 2.19$\pm$0.65  \\ 
  TPR@0.01 & 1.56$\pm$0.57 & 2.86$\pm$0.72 & 3.73$\pm$0.55 & 1.85$\pm$0.58  \\ 
  CVOL@0.01 & 1.39$\pm$0.65 & 2.96$\pm$0.56 & 3.81$\pm$0.45 & 1.83$\pm$0.68  \\ \hline
 \end{tabular}
 \caption{Means and standard deviations of algorithm ranks using different measures, UMAP datasets, 0\% training contamination.} 
 \label{tab:model_ranks_umap} 
\end{table}
